Invariants of Self-Intersected N-Periodics in the Elliptic Billiard

We study self-intersected N-periodics in the elliptic billiard, describing new facts about their geometry (e.g., self-intersected 4-periodics have vertices concyclic with the foci). We also check if some invariants listed in "Eighty New Invariants of N-Periodics in the Elliptic Billiard" (2020), arXiv:2004.12497, remain invariant in the self-intersected case. Toward that end, we derive explicit expressions for many low-N simple and self-intersected cases. We identify two special cases (one simple, one self-intersected) where a quantity prescribed to be invariant is actually variable.

==> app/310_app_regular_polys.tex <==
\begin{align*}
    J=&  \frac{\sqrt{2}}{2a}\sqrt{1-\cos(2\pi/N)}
\\
    L=& 2 N a^2 J \\
    k_{101}=& JL-N \\
    k_{102}=&  \cos^N \left[  \frac {\pi\, \left( N-2 \right) }{N}\right]   =\left(\frac{J L}{N}-1\right) ^{N}
\\
    k_{103}=& ...\\
    k_{104}=& ... \\
    k_{105}=& ... \\
    k_{106}=& ... \\
    k_{107}=& ... \\
    k_{108}=& 
\end{align*}

==> app/320_app_invariant_numeric.tex <==
The tables below present values for $J$, $L$, $J L$, and $k_i,i=1{\ldots}8$, $N=3{\ldots}12$ for a few values of $a/b$, obtained from numerical simulation. Numbers show approximated to 3 decimals.

\subsection{$a/b=1$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.866 & 0.707 & 0.588 & 0.5 & 0.434 & 0.383 & 0.342 & 0.309 & 0.282 & 0.259 \\
 \text{L} & 5.196 & 5.657 & 5.878 & 6 & 6.074 & 6.123 & 6.156 & 6.18 & 6.198 & 6.212 \\
 \text{JL} & 4.5 & 4 & 3.455 & 3 & 2.636 & 2.343 & 2.106 & 1.91 & 1.746 & 1.608 \\
 k_{101} & 1.5 & 0 & -1.545 & -3 & -4.364 & -5.657 & -6.894 & -8.09 & -9.254 & -10.392 \\
 k_{102} & 0.125 & 0 & -0.003 & 0.016 & -0.037 & 0.062 & -0.091 & 0.12 & -0.149 & 0.178 \\
 k_{103} & 4 & \text{n/a} & 1.528 & \text{n/a} & 1.232 & \text{n/a} & 1.132 & \text{n/a} & 1.086 & \text{n/a} \\
 k_{104} & -1.5 & -4 & -4.045 & -3 & -1.558 & 0 & 1.563 & 3.09 & 4.57 & 6\\
 k_{105} & 0.125 & \text{n/a} & 0.347 & \text{n/a} & 0.482 & \text{n/a} & 0.571 & \text{n/a} & 0.635 & \text{n/a} \\
 k_{106} & \text{n/a} & 8 & \text{n/a} & 9 & \text{n/a} & 9.373 & \text{n/a} & 9.549 & \text{n/a} & 9.646 \\
 k_{107} & \text{n/a} & 0.5 & \text{n/a} & \text{n/a} & \text{n/a} & 0.622 & \text{n/a} & \text{n/a} & \text{n/a} & 0.707 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.16 & \text{n/a} & \text{n/a} & \text{n/a} & 1.826 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=1.25$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.752 & 0.625 & 0.522 & 0.444 & 0.386 & 0.341 & 0.305 & 0.275 & 0.251 & 0.231 \\
 \text{L} & 5.916 & 6.403 & 6.644 & 6.778 & 6.86 & 6.913 & 6.95 & 6.977 & 6.996 & 7.011 \\
 \text{JL} & 4.449 & 4 & 3.465 & 3.012 & 2.648 & 2.355 & 2.117 & 1.92 & 1.756 & 1.617 \\
 k_{101} & 1.449 & 0 & -1.535 & -2.988 & -4.352 & -5.645 & -6.883 & -8.08 & -9.244 & -10.383 \\
 k_{102} & 0.112 & 0 & -0.003 & 0.015 & -0.036 & 0.061 & -0.09 & 0.119 & -0.148 & 0.176 \\
 k_{103} & 4.451 & \text{n/a} & 1.546 & \text{n/a} & 1.238 & \text{n/a} & 1.135 & \text{n/a} & 1.088 & \text{n/a} \\
 k_{104} & -1.449 & -4 & -4.035 & -2.988 & -1.551 & 0 & 1.557 & 3.08 & 4.556 & 5.984 \\
 k_{105} & 0.112 & \text{n/a} & 0.342 & \text{n/a} & 0.479 & \text{n/a} & 0.569 & \text{n/a} & 0.633 & \text{n/a} \\
 k_{106} & \text{n/a} & 12.5 & \text{n/a} & 14.043 & \text{n/a} & 14.632 & \text{n/a} & 14.912 & \text{n/a} & 15.066 \\
 k_{107} & \text{n/a} & 0.476 & \text{n/a} & \text{n/a} & \text{n/a} & 0.621 & \text{n/a} & \text{n/a} & \text{n/a} & 0.706 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.211 & \text{n/a} & \text{n/a} & \text{n/a} & 1.836 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=1.5$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
\hline
 \text{J} & 0.648 & 0.555 & 0.467 & 0.4 & 0.348 & 0.308 & 0.275 & 0.249 & 0.227 & 0.209 \\
 \text{L} & 6.738 & 7.211 & 7.459 & 7.6 & 7.687 & 7.743 & 7.783 & 7.811 & 7.832 & 7.848 \\
 \text{JL} & 4.363 & 4 & 3.487 & 3.04 & 2.676 & 2.382 & 2.143 & 1.944 & 1.779 & 1.638 \\
 k_{101} & 1.363 & 0 & -1.513 & -2.96 & -4.324 & -5.618 & -6.857 & -8.056 & -9.221 & -10.362 \\
 k_{102} & 0.091 & 0 & -0.003 & 0.014 & -0.034 & 0.059 & -0.087 & 0.115 & -0.144 & 0.172 \\
 k_{103} & 5.515 & \text{n/a} & 1.587 & \text{n/a} & 1.251 & \text{n/a} & 1.142 & \text{n/a} & 1.092 & \text{n/a} \\
 k_{104} & -1.363 & -4 & -4.012 & -2.96 & -1.535 & 0 & 1.543 & 3.056 & 4.525 & 5.948 \\
 k_{105} & 0.091 & \text{n/a} & 0.333 & \text{n/a} & 0.472 & \text{n/a} & 0.564 & \text{n/a} & 0.628 & \text{n/a} \\
 k_{106} & \text{n/a} & 18 & \text{n/a} & 20.16 & \text{n/a} & 21.028 & \text{n/a} & 21.444 & \text{n/a} & 21.674 \\
 k_{107} & \text{n/a} & 0.426 & \text{n/a} & \text{n/a} & \text{n/a} & 0.618 & \text{n/a} & \text{n/a} & \text{n/a} & 0.704 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.338 & \text{n/a} & \text{n/a} & \text{n/a} & 1.86 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=2$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
\hline
 \text{J} & 0.496 & 0.447 & 0.386 & 0.333 & 0.292 & 0.259 & 0.232 & 0.21 & 0.192 & 0.177 \\
 \text{L} & 8.531 & 8.944 & 9.189 & 9.333 & 9.424 & 9.485 & 9.526 & 9.557 & 9.579 & 9.597 \\
 \text{JL} & 4.228 & 4 & 3.542 & 3.111 & 2.75 & 2.454 & 2.21 & 2.008 & 1.838 & 1.694 \\
 k_{101} & 1.228 & 0 & -1.458 & -2.889 & -4.25 & -5.546 & -6.79 & -7.992 & -9.162 & -10.306 \\
 k_{102} & 0.057 & 0 & -0.002 & 0.012 & -0.03 & 0.053 & -0.079 & 0.106 & -0.134 & 0.161 \\
 k_{103} & 8.757 & \text{n/a} & 1.702 & \text{n/a} & 1.287 & \text{n/a} & 1.161 & \text{n/a} & 1.103 & \text{n/a} \\
 k_{104} & -1.228 & -4 & -3.954 & -2.889 & -1.495 & 0 & 1.508 & 2.994 & 4.443 & 5.853 \\
 k_{105} & 0.057 & \text{n/a} & 0.309 & \text{n/a} & 0.455 & \text{n/a} & 0.549 & \text{n/a} & 0.616 & \text{n/a} \\
 k_{106} & \text{n/a} & 32 & \text{n/a} & 35.556 & \text{n/a} & 37.183 & \text{n/a} & 37.986 & \text{n/a} & 38.434 \\
 k_{107} & \text{n/a} & 0.32 & \text{n/a} & \text{n/a} & \text{n/a} & 0.612 & \text{n/a} & \text{n/a} & \text{n/a} & 0.697 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 3.732 & \text{n/a} & \text{n/a} & \text{n/a} & 1.927 & \text{n/a} & \text{n/a} \\
\end{array}
$$

\subsection{$a/b=3$}

$$
\scriptsize
\begin{array}{r|rrrrrrrrrr}
 \text{N} & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\
 \hline
 \text{J} & 0.333 & 0.316 & 0.283 & 0.25 & 0.221 & 0.198 & 0.178 & 0.162 & 0.148 & 0.137 \\
 \text{L} & 12.343 & 12.649 & 12.863 & 13 & 13.09 & 13.151 & 13.194 & 13.225 & 13.249 & 13.267 \\
 \text{JL} & 4.108 & 4. & 3.643 & 3.25 & 2.899 & 2.602 & 2.352 & 2.143 & 1.965 & 1.814 \\
 k_{101} & 1.108 & 0 & -1.357 & -2.75 & -4.101 & -5.398 & -6.648 & -7.857 & -9.035 & -10.186 \\
 k_{102} & 0.027 & 0 & -0.001 & 0.009 & -0.023 & 0.042 & -0.065 & 0.089 & -0.114 & 0.139 \\
 k_{103} & 18.604 & \text{n/a} & 1.977 & \text{n/a} & 1.372 & \text{n/a} & 1.203 & \text{n/a} & 1.129 & \text{n/a} \\
 k_{104} & -1.108 & -4 & -3.84 & -2.75 & -1.417 & 0 & 1.438 & 2.868 & 4.277 & 5.658 \\
 k_{105} & 0.027 & \text{n/a} & 0.263 & \text{n/a} & 0.419 & \text{n/a} & 0.519 & \text{n/a} & 0.59 & \text{n/a} \\
 k_{106} & \text{n/a} & 72 & \text{n/a} & 78.75 & \text{n/a} & 82.714 & \text{n/a} & 84.799 & \text{n/a} & 85.989 \\
 k_{107} & \text{n/a} & 0.18 & \text{n/a} & \text{n/a} & \text{n/a} & 0.595 & \text{n/a} & \text{n/a} & \text{n/a} & 0.684 \\
 k_{108} & \text{n/a} & \text{n/a} & \text{n/a} & 4.874 & \text{n/a} & \text{n/a} & \text{n/a} & 2.082 & \text{n/a} & \text{n/a} \\
\end{array}
$$
